FDP control in multivariate linear models using the bootstrap

In this article we develop a method for performing post hoc inference of the False Discovery Proportion (FDP) over multiple contrasts of interest in the multivariate linear model. To do so we use the bootstrap to simulate from the distribution of the null contrasts. We combine the bootstrap with the post hoc inference bounds of Blanchard (2020) and prove that doing so provides simultaneous asymptotic control of the FDP over all subsets of hypotheses. This requires us to demonstrate consistency of the multivariate bootstrap in the linear model, which we do via the Lindeberg Central Limit Theorem, providing a simpler proof of this result than that of Eck (2018). We demonstrate, via simulations, that our approach provides simultaneous control of the FDP over all subsets and is typically more powerful than existing, state of the art, parametric methods. We illustrate our approach on functional Magnetic Resonance Imaging data from the Human Connectome project and on a transcriptomic dataset of chronic obstructive pulmonary disease.

==> main_body_secondhalf.tex <==
As the follow theorem demonstrates, the step-down approach controls the joint error rate and therefore provides simultaneous FDP control.
\vspace{0.08cm}
\begin{theorem}\label{thm:stepdown}
	Let $ \hat{H}_n $ be the set generated by applying Algorithm \ref{Alg:stepdown}. Then 
	\begin{equation*}
	\lim_{n \rightarrow \infty} \lim_{B \rightarrow \infty} \mathbb{P}\left( f_{n, \mathcal{N}}(T_n) < \lambda^*_{\alpha,n,B}(\hat{H}_n) \right) \leq \alpha.
	\end{equation*}
	In particular, for $ H \subset \mathcal{H}, $ letting $ \mybar{V}_{\alpha, n,B}(H) = |H| \wedge \min_{1 \leq k \leq K} (|H \setminus R_k(\lambda^*_{\alpha,n,B}(\hat{H}_n))| + \zeta_k), $ it follows that 
	\begin{equation*}
	\lim_{n \rightarrow \infty}\lim_{B \rightarrow \infty}\mathbb{P}\left(|H \cap \mathcal{N}| \leq \mybar{V}_{\alpha, n,B}(H),\,\, \forall H \subset \mathcal{H}  \right) \leq 1-\alpha.
	\end{equation*}
\end{theorem}

\begin{remark}
	The results in this subsection and the one previous have been stated for two-sided $ p $-values however they also hold for one-sided $ p $-values without change. All that is required to show this is to re-define $ p^n_{(k:H)}(T) $ as the $ k $th minimum value in the set \begin{equation*}
	\left\lbrace 1 - \Phi_{n-r}(T_l(v)): (l,v) \in H, l \leq \text{dim}(T(v))  \right\rbrace.
	\end{equation*}
\end{remark}

% Test conditioning
\if\biometrika0
\input{./ARI.tex}
\fi

\section{Simulation Results}\label{SS:simulations}
\subsection{Simulation Setup}\label{SS:simsetup}
In order to assess empirically that our method correctly controls the false positive rate we run numerical simulations. We create the noise in these simulations by generating 2D stationary Gaussian random fields with sizes $ [25, 25] $, $ [50,50] $ and $[100,100]$ which are formed by smoothing white noise with a Gaussian kernel with full width at half maximum in $ \left\lbrace 0, 4, 8 \right\rbrace $ (in pixel units), accounting for edge effects to ensure stationarity (see e.g. \cite{Davenport2021Ravi}), and scaled so that the variance is 1 everywhere.

We let the total number of subjects $ n $ range from $ 20 $ to $ 100 $. For each $ n $, smoothness level, image size and $ \pi_0 \in \left\lbrace 0.5, 0.8, 0.9, 1 \right\rbrace$, we run 5000 simulations - each with 1000 bootstraps - to test the false positive rate. For each simulation we do the following. First we generate $ n $ Gaussian random fields $ \epsilon_1, \dots, \epsilon_n $ as described above and add signal to them (as detailed in the next paragraph). We then randomly divide these images into 3 disjoint groups: $ G_1, G_2, G_3 \subset \left\lbrace 1, \dots, n \right\rbrace $ - performing assignment to each group with equal probability (we eliminate assignments where a given group has no entries). We test for the difference between the first and the second group and between the second and the third group - giving us two contrasts to differentiate between. We thus, in total, test $ 5000 $ hypotheses for the 50 by 50 scenario and $20000$ for the 100 by 100 case.

We vary the amount of signal in the datasets as follows. Given a proportion $ \pi_0 $ we randomly choose a subset $ \mathcal{N} $ of size $ \pi_0\left| \mathcal{H} \right| $ of the hypotheses to be null (which is thus different in each simulation) and add signal to ensure that the remainder are non-null. To do so, for $ 1 \leq i \leq n, $ and each $ v \in \mathcal{V} $, we set 
\begin{equation*}
Y_i(v) = 1[i \in G_2, (1,v) \not\in \mathcal{N}]  + 1[i \in G_3, (1,v) \not\in \mathcal{N}] + 1[i \in G_3, (2,v) \not\in \mathcal{N}] + \epsilon_i(v).
\end{equation*}
This ensures that the power of the test to detect a difference at $ h $ is equal for any $ h \in \mathcal{N}^C $. If $ \pi_0 = 1 $ then all hypotheses are null. An example realisation is shown in Figure \ref{simimages}.

In the next subsections we compare our bootstrap procedures to the two parametric alternatives, described in Section~\ref{sec:param-approaches}, in terms of false positive control, and power. 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=0.4\textwidth]{./Figures/SimulationImages/signal.png}
		\includegraphics[width=0.4\textwidth]{./Figures/SimulationImages/realisation.png}
	\end{center}
\caption{Illustrating the simulation setup for a domain of size [25,25] and a smoothness of 4 pixels. Left: the signal for the first contrast. Right: a realisation of one of the subjects in $ G_2. $}\label{simimages}
\end{figure}

\subsection{False Positive control}\label{JERFPR}
In each simulation setting, for $ 1 \leq j \leq 5000 $, we calculate a test statistic random field $ T_{n}^{(j)} $ and obtain $ \lambda $ thresholds for the single-step bootstrap, step-down bootstrap, Simes and ARI methods based on the data as described in Section \ref{S:LMJER}, where we have used 100 bootstraps for the non-parametric procedures. For each method we obtain $ \lambda $-thresholds $ \lambda_1, \dots, \lambda_{5000} $ allowing us to estimate the joint error rate via the statistic $ \frac{1}{5000}\sum_{j = 1}^{5000} 1[f_{n, \mathcal{N}}(T_{n}^{(j)}) \leq \lambda_j] $ which we refer to as the \textbf{empirical JER}. Note that here $ 1[\cdot] $ denotes the indicator function. 

The results are displayed in Figure \ref{fig:fpr50}. 
%
The results for the bootstrap methods are shown in blue whilst those for the parametric methods are shown in red. 
%
The solid lines indicate the step-down methods (i.e. ARI and the step-down bootstrap). 
%
These plots demonstrate that, given a reasonable number of subjects, the joint error rate of the bootstrap procedures converges to the nominal level (in this case 0.1). 
%
The parametric procedures are valid in all settings.
%
However, the parametric procedure control the joint error rate at a rate that is substantially below the nominal level under dependence (i.e. when the applied smoothing is non-zero), while the bootstrap approaches have a tighter control of the joint error rate.
%
Moreover, the single-step procedures are slightly more conservative than their parametric counterparts. 
%
This difference increases as $ \pi_0 $ decreases. See the following section for further details on the effect of $ \pi_0 $.
%
\begin{figure}[h!]
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_0_pi0_100.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_4_pi0_100.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_8_pi0_100.pdf}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_0_pi0_90.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_4_pi0_90.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_8_pi0_90.pdf}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_0_pi0_80.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_4_pi0_80.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_8_pi0_80.pdf}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_0_pi0_50.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_4_pi0_50.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering
		\includegraphics[width=\textwidth]{./Figures/EJERFinalPlots/JER_dim_50_fwhm_8_pi0_50.pdf}
	\end{subfigure}
	\caption{Comparing the empirical joint error rate across methods for the simulation setting described in Section \ref{SS:simsetup} for $ \alpha = 0.1 $. The bootstrap procedures typically provide tighter control of the joint error rate than the parametric ones, except under independence. The bootstrap methods are shown in blue whilst the parametric methods are shown in red. The solid lines indicate the step-down methods. The uncertainty bands provide 95\% marginal confidence bands based on the normal approximation to the binomial distribution.}\label{fig:fpr50}
\end{figure}

%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width=0.47\textwidth]{./Figures/Ejoint error rate_nsubj_dim/joint error rate_dim_50_contrastno_1.pdf}
%	\includegraphics[width=0.47\textwidth]{./Figures/Ejoint error rate_nsubj_dim/joint error rate_dim_150_contrastno_1.pdf}
%	\end{center}
%\caption{JER control vs the number of subjects and smoothness. We have calculated the empirical joint error rate for evaluating the joint error rate in a setting where we are testing 2 contrasts of differences between 3 groups. The error reaches the nominal rate of 0.1 given sufficiently many subjects. This convergence is quicker at higher levels of smoothness.}\label{fig:simresults}
%\end{figure}

\subsection{Power}
In this section we compare the power of the various methods in the simulation setting described in Section \ref{SS:simsetup} in the case where the applied full width at half maximum is 4 pixels. We have chosen to focus on this level of smoothness because it represents a realistic level of applied smoothness and illustrates the benefits that can be achieved when using the bootstrap under dependence.

Here we shall use a notion of power originally proposed in \cite{Blanchard2020} to compare the ability of joint error rate controlling procedures to detect signal. Given a set $ R \subset \mathcal{H} $, define
\begin{equation*}
\text{Pow}(R) := \mathbb{E}\left[ \frac{|R| - \mybar{V}(R)}{\left| R \cap (\mathcal{H} \setminus \mathcal{N}) \right|} \middle| \left| R \cap (\mathcal{H} \setminus \mathcal{N}) \right| > 0\right]
\end{equation*}
where $ \mybar{V} $ is defined as in equation \ref{eq:Vbar}. Here we consider the following choices of $ R $ with which we compare the power (as in \cite{Blanchard2020}). 1) $ R = \mathcal{H} $ and 2) Taking $ R $ to be the hypotheses of $ \mathcal{H} $ which are rejected by the Benjamini Hochberg procedure, applied to the $ p $-values $ \left\lbrace p_{n,l}(v): (l, v) \in \mathcal{H}  \right\rbrace $, at a level $ 0.05 $. Note that, unlike in \cite{Blanchard2020}, no additional level of randomness in the choice of the sets in 2) is prescribed. We also consider taking $ R = \left\lbrace (l, v): p_{n, l}(v) \leq 0.05  \right\rbrace$, however the results are similar in nature to scenario 1 from above and so have been regulated to the supplementary material. The results for  cases 1) and 2) are illustrated graphically in Figure \ref{fig:power}.

\begin{figure}[h!]
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_50_powertype_0.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_80_powertype_0.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_90_powertype_0.png}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_50_powertype_4.png}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_80_powertype_4.png}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.32\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./Figures/Power/dim_5050_pi0_90_powertype_4.png}
	\end{subfigure}
\hfill
	\caption{Plotting the power of the different methods against the numbers of a subjects. The power for setting 1 (i.e. $ R $ = $ \mathcal{H} $) is shown in the top row and the power for setting 2 (i.e. taking $ R $ to be the Benjamini-Hochberg rejection set) is shown in the bottom row. In this setting the bootstrap methods typically have a larger power than the parametric methods (even if the step-down is not used).}\label{fig:power}
\end{figure}

From these plots we can see that overall the bootstrap based approaches have a higher power than the parametric ones. The power of ARI only becomes comparable (or higher) to that of the bootstrap in the extreme scenario ($ \pi_0 = 0.5 $) given a large enough sample size. Additionally the bootstrap is not robust at the smallest sample size considered (i.e. $ n = 10 $) where the bootstrap is conservative. It is worth noting here, that in typical high-dimensional applications (neuroimaging, genetics)  $\pi_0 > 0.9$ and $ n $ is often substantially greater than $ 20. $

The lower the value of $ \pi_0 $, the greater the increase in power that is obtained by using the step-down algorithms. ARI is always more powerful than Simes by construction. In the relatively sparse scenarios (i.e. $ \pi_0 \geq 0.8 $) they have a very similar power however for $ \pi_0 = 0.5 $, ARI provides a marked improvement over Simes. The bootstrap step-down always improves on the standard bootstrap approach though the difference is not particularly large: even in the $ \pi = 0.5 $ scenario this is increase is relatively small. The similarity of the standard and step-down procedures, for both the parametric and bootstrap methods, is consistent with the results obtained on real data which are described in the next subsections.

%Comments:
%\begin{itemize}
%\item Overall boostrap $>$ parametric, except in non-sparse scenarios ($\pi_0=0.5$) with large sample size 
%\item ARI always $>$ Simes by construction; in the relatively sparse scenarios ($\pi_0 \geq 0.8$), very close to each other (consistent with results obtained on real data and described in the next subsections)
%\item in the extreme case where $\pi_0=0.5$ ARI is better than Simes for large enough sample sizes; in this case ARI can be competitive with the bootstrap, but in typical high-dimensional applications (neuroimaging, genetics)  $\pi_0 > 0.9$
%\item bootstrap can be conservative for very low sample sizes
%\end{itemize}

\section{Real Data results}
\subsection{Neuroimaging data application}\label{SS:neuroapp}
We have 3D functional Magnetic Resonance Imaging data from $ n = 386 $ unrelated subjects, who performed a working memory task, from the Human Connectome Project. After pre-processing (described in Section XXX) we obtain a contrast image for each subject. We fit a linear model to these images including sex, height, weight, BMI, two different measures of blood pressure, handedness and IQ (measured using the PMAT24\_A\_CR test score). We consider sex and IQ as a variables of interest. We obtain test-statistic contrasts for sex and IQ and a $ p $-value at each voxel for each contrast. We form clusters using a cluster defining threshold on the $ p $-values of $ p = 0.001 $, with each cluster being a contiguous set of voxels above the threshold (clusters are defined separately for each contrast of interest). We obtain bounds on the true discovery proportion as described in Section \ref{SS:JERcontrol}.

Within each cluster above the threshold we use our bootstrap framework to provide a lower bound on the proportion of active voxels within each cluster. We find a number of clusters with a relatively large proportion of active voxels in different regions of the brain for the contrast of IQ. For the contrast of sex only a single cluster has a non-zero lower bound on the number of true positives. The results for the IQ contrast are shown graphically in the upper panel of Figure \ref{fig:realdata}. The results for the sex contrast are shown in Section XXX. The bounds provided using the step-down bootstrap procedure are the same as the single-step version in this example.

We compare to the result of using the approach of \cite{Rosenblatt2017} and see that the non-parametric approach results in a higher bound on the number of active voxels. The results of using all resolutions inference are almost identical to those of the Simes procedure, which is not surprising given the sparsity of the signal. For completeness the same plot, but for the Simes procedure, is shown in Section XXX.

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=\textwidth]{./Figures/HCP/TDP_boot_iq_sex_1.pdf}
		\includegraphics[width=\textwidth]{./Figures/HCP/TDP_ari_iq_sex_1.pdf}
	\end{center}
\caption{TDP bounds within clusters for the contrast for IQ in the linear regression model fit to the HCP data. Each cluster is shaded a single colour which is the lower bound on the TDP. The upper panel gives the TDP bounds within each cluster provided by the bootstrap procedure. The lower panel gives the bounds provided by using ARI. The bounds given by the bootstrap are larger (as indicated by the light colours) indicating that the method is more powerful. Note that these images are 2D slices through the 3D brain and so voxels that are part of the same cluster are not necessarily connected.}\label{fig:realdata}
\end{figure}


\begin{figure}[h]
	\begin{center}
		\includegraphics[width=0.48\textwidth]{./Figures/HCP/TDP_cluster_plot_iq_sex.pdf}
		\includegraphics[width=0.48\textwidth]{./Figures/HCP/TP_cluster_plot_iq_sex.pdf}
	\end{center}
\caption{Comparing the TDP and TP lower bounds across clusters for the different methods. The bootstrap lower bounds are consistently higher than the parametric methods. Clusters are organized from left to right in terms of their size. Only one cluster for the sex contrast is found: this is the 2nd smallest cluster overall with a TP lower bound of 1 voxel. The sizes and bounds of the clusters in the IQ contrast are larger. For the largest cluster we are able to conclude that it contains 908 true positives using the bootstrap.}\label{fig:tdphcpplots}
\end{figure}

\subsection{Transcriptomic data application}\label{SS:trans}
In this section, we illustrate the application of our methods to a specific gene expression data set. 
%
Gene expression studies use microarray or sequencing biotechologies in order to measure the activity (or ``expression level'') of a large number of genes simultaneously. 
%
We focus on a study of chronic obstructive pulmonary disease (COPD), \cite{bahr2013peripheral}, whose main goal was to identify genes whose expression level is significantly associated with lung function. 
%
In order to do this, the authors fit a linear model for this association for each gene, while controlling for the following covariates: age, sex, body mass index, parental history of COPD, and two smoking variables (smoking status and pack-years).
%
The number of subjects is $n = 135$ while the number of genes is $V = 12,531$, leading to a large-scale multiple testing problem. 
%
Using the Benjamini-Hochberg method to controlling the FDR at the $5\%$ level, $1,745$ genes were found to be significantly associated.

We fit this linear model to the data, regressing the gene level data against the controlled covariates and lung function and considering a single contrast for lung function. We performed 1000 bootstraps and used these to obtain $ \lambda^*_{\alpha, 135, 1000} = 0.22 $, where we took $ \alpha = 0.1. $ This allows us to provide a $ \alpha $-level simultaneous bounds on the number of true positives within any specified set of genes via \eqref{eq:Vbar}. In particular it allows us to conclude (with $90\%$ confidence) that at least 1,354 of the 1,745 genes within the Benjamini-Hochberg significance set are active. The stepdown bootstrap provides the same bound as the single step version in this case. Simes and ARI provide lower bounds on the number of true positives in this set of 917 and 966 respectively, which are substantially lower than the bootstrap bounds.

In the absence of prior information on genes, a natural idea is to rank them by decreasing statistical significance. 
%
Post hoc methods provide upper confidence curves on the proportion of true positives among the most significant genes.  
%
Such curves are displayed in Figure \ref{fig:fdpplot}, where the blue lines correspond to our proposed single step (dashed lines) and step-down (solid lines) bootstrap-based methods, and the red lines correspond to the state-of-the-art parametric approaches described in Section \ref{sec:param-approaches}, that is the original Simes bound of \cite{Goeman2011} and the ARI bound of \cite{Rosenblatt2018}.
%
These results are consistent with the numerical experiments of Section \ref{SS:simulations}.
%
First, the bootstrap method yields post hoc bounds that are substantially more informative that their parametric counterpart.
%
Second, the difference between single-step methods (dashed lines) and their step-down or $\pi_0$-adaptive counterpart (solid lines) is very small, which is consistent with the fact that the signal is expected to be small in such genomic data sets, corresponding to $\pi_0$ close to $1$. For the bootstrap there is no difference between the single step and step-down approach in this case.

% VOLCANO PLOT description.
A widely used approach in differential expression studies is to select genes based on the conjunction of a threshold on the $p$-values and a threshold on its effect size \citep{Cui2003}.
%
\cite{Ebrahimpoor2020} have recently noted that this type of double selection can lead to inflated numbers of false discoveries when used in conjunction of FDR-based multiple testing corrections, whereas post hoc inference is by construction robust against this issue.
%
The use of our proposed post hoc bounds in this context is illustrated in the Volcano plot in Figure \ref{fig:volcano} \citep{Cui2003}.
%
In this plot, each gene is represented in two dimensions by estimates of its effect size ($x$ axis, also kown as ``fold change'' in genomics) and significance ($y$ axis), in a logarithmic scale.
%
Figure~\ref{fig:volcano} illustrates a particular selection, corresponding to the genes whose $p$-value is below $0.001$ and whose effect size is above $0.5$.
%
Our bootstrap-based bound  ensures that with probability $1-\alpha = 90\%$, among these $546$ genes, at least $490$ are true positives, corresponding to a FDP below $0.1$. 
%
Importantly, the $p$-value and effect size thresholds can be chosen post hoc, and multiple such choices can be made without compromising the statistical coverage of the associated bound.
%
For example, the bounds associated to the gene subsets with positive and negative effect size are also displayed in Figure~\ref{fig:volcano}. 

\begin{figure}[h]
	\centering\includegraphics[width=0.8\textwidth]{./Figures/Genetics_Dataset/fdpplot_3000.pdf}
	\centering\includegraphics[width=0.8\textwidth]{./Figures/Genetics_Dataset/fdpplot_1000.pdf}
	\caption{False discovery proportion and true positive (TP) plots for the transcriptomic dataset. In the upper panels, for $ k = 1, \dots, 3000 $, upper bounds on the FDP and lower bounds on the TP are provided by each of the methods for the sets comprised of the hypotheses with the $ k $ smallest $ p $-values. The grey vertical dashed line indicates the Benjamini-Hochberg rejection set. The lower panels provide a zoomed in version same plot for for the $ 1000 $ smallest $ p $-values. The bootstrap methods provide substantially better bounds than the parametric ones. ARI slightly improves on Simes while the step-down bootstrap is indistinguishable from the single step bootstrap approach in this setting.}\label{fig:fdpplot}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.7\textwidth]{./Figures/Genetics_Dataset/volcano_plot.png}
	\caption{A volcano plot for the $ p $-values for the transcriptomic data. For each gene this plots the estimated contrast effect size (labelled as fold change and corresponding to $ c^T\hat\beta_{135} $ where $ c$ is the contrast vector for COPD) against the $ p $-value, where both are measured in log scale. Two regions (shown in red) are selected containing the genes whose $ p $-values are less than $ 10^{-3} $ and for which the absolute fold change is greater than $ 10^{0.4} $.  Appling the bootstrap to control the joint error rate at a level 0.1, out of the 546 genes selected at least 490 are true positives.}\label{fig:volcano}
\end{figure}

